Delineating Bone Surfaces in B-Mode Images Constrained by Physics of Ultrasound Propagation

Bone surface delineation in ultrasound is of interest due to its potential in diagnosis, surgical planning, and post-operative follow-up in orthopedics, as well as the potential of using bones as anatomical landmarks in surgical navigation. We herein propose a method to encode the physics of ultrasound propagation into a factor graph formulation for the purpose of bone surface delineation. In this graph structure, unary node potentials encode the local likelihood for being a soft tissue or acoustic-shadow (behind bone surface) region, both learned through image descriptors. Pair-wise edge potentials encode ultrasound propagation constraints of bone surfaces given their large acoustic-impedance difference. We evaluate the proposed method in comparison with four earlier approaches, on in-vivo ultrasound images collected from dorsal and volar views of the forearm. The proposed method achieves an average root-mean-square error and symmetric Hausdorff distance of 0.28mm and 1.78mm, respectively. It detects 99.9% of the annotated bone surfaces with a mean scanline error (distance to annotations) of 0.39mm.

==> featExtractionTime_pie.tex <==
\begin{figure}%[!t]
\centering
\includegraphics[trim = 0mm 0mm 0mm 0mm, clip, width=\linewidth]{./featTime3.png}
\caption{
The pie chart (left) depicts the relative computation times of the union of the most important 7 feature groups for both classifiers \textbf{S}~\&~\textbf{T}.
Although it is among the top feature groups, computation time of CW local statistics is not displayed due to being negligibly low compared to the rest. 
Note that log-shadowing and shadowing features are grouped as (log-/Shadowing) as they can be computed together with little overhead.
(Right) Mean computation times of feature groups with $>$30\,ms computation. 
}
\label{fig:featExtractionTime_pie}
\end{figure}

==> featureMaps.tex <==
\begin{figure}%[!t]
\centering
\begin{tabular}{l}
    \includegraphics[width=\textwidth]{./featMapsr1.png}\\
    [-3.ex]{\tiny%
    \hspace{0.9cm} image \hspace{1.5cm} confidence map \hspace{0.6cm} Rayleigh fit error \hspace{0.9cm} patch variance \hspace{1.0cm} patch median%
    }\\
    \includegraphics[width=\textwidth]{./featMapsr2.png}\\
    [-3ex]{\tiny%
    $1^{st}$ ord.\ CW local stat.\ \hspace{0.01cm} $2^{nd}$ ord.\ CW local stat.\ \hspace{0.7cm} LBP \hspace{1.5cm} extended LBP \hspace{0.7cm} CW cumulative mean%
    }\\
    \includegraphics[width=\textwidth]{./featMapsr3.png}\\
    [-3.ex]{\tiny%
    \hspace{0.1cm} CW cumulative std. \hspace{0.5cm} curvature map \hspace{1.0cm} Haar features \hspace{0.8cm} Attenuation feature \hspace{0.40cm} Shadowing feature%
    }
\end{tabular}
\caption{For an example US image, a representative subset of corresponding feature maps are shown.}
\label{fig:featureMaps}
\end{figure}
